Overestimation, Overfitting, and Plasticity in Actor-Critic: the Bitter Lesson of Reinforcement Learning

Recent advancements in off-policy Reinforcement Learning (RL) have significantly improved sample efficiency, primarily due to the incorporation of various forms of regularization that enable more gradient update steps than traditional agents. However, many of these techniques have been tested in limited settings, often on tasks from single simulation benchmarks and against well-known algorithms rather than a range of regularization approaches. This limits our understanding of the specific mechanisms driving RL improvements. To address this, we implemented over 60 different off-policy agents, each integrating established regularization techniques from recent state-of-the-art algorithms. We tested these agents across 14 diverse tasks from 2 simulation benchmarks, measuring training metrics related to overestimation, overfitting, and plasticity loss -- issues that motivate the examined regularization techniques. Our findings reveal that while the effectiveness of a specific regularization setup varies with the task, certain combinations consistently demonstrate robust and superior performance. Notably, a simple Soft Actor-Critic agent, appropriately regularized, reliably finds a better-performing policy within the training regime, which previously was achieved mainly through model-based approaches.

==> old_text.tex <==
We list our contributions in the bullets below:

% \begin{enumerate}
%     \item We report on the results of over 12k training runs testing 64 combinations of critic, network and plasticity regularization techniques that were used in recent SOTA algorithms. We systemically study the synergies and robustness of each regularization technique on a variety of complex locomotion and manipulation tasks. 
%     \item We find that applying a suite of well-known regularization techniques in conjunction with methods for plasticity preservation largely alleviates the value estimation problem, and allows \textit{for not using critic regularization}. In particular, we find that in such network/plasticity regularized agents using critic regularization often leads to statistically significant performance degradation.
%     \item We find that applying certain regularization methods to simple Soft Actor-Critic leads to algorithms that reliably solve the task from dog domain, which were previously unsolved by model-free approaches
%     \item We perform an extensive empirical study measuring the impact of different regularization techniques on overestimation, overfitting and plasticity of the resulting agent. In contrast to previous work, we find ...
%     \item Furthermore, we study the impact of overestimation, overfitting and plasticity of the resulting agent performance. We find that the instrument for measuring plasticity is ... 
% \end{enumerate}

\begin{enumerate}
    \item We find that applying a suite of well-known network regularization techniques in conjunction with methods preventing plasticity loss largely alleviates the value estimation problem and allows \textit{for not using critic regularization}. In particular, we find that in such network/plasticity regularized agents using critic regularization often leads to significant performance degradation.
    \item Building upon the insights from the preceding analysis, we observe that incorporating specific regularization methods into the basic Soft Actor-Critic framework yields state-of-the-art outcomes in dog domain tasks within model-free approaches. %We find that applying certain regularization methods to simple Soft Actor-Critic leads to algorithms that reliably solve the task from the dog domain, which were previously unsolvable by model-free approaches. \michalb{Połączyć z punktem pierwszym - Following the analysis from contrib 1...} \michalb{Write explicitly SOTA on model-free, proprioceptive (może być tylko w abstrakcie)}
    %\item We perform an extensive empirical study measuring the impact of different regularization techniques on overestimation, overfitting and plasticity on the SAC agent. We report the synergies and robustness of each regularization technique on a variety of complex locomotion and manipulation tasks. In contrast to previous work, we find ...
    \item We perform an extensive empirical study measuring the correlation of Overestimation, Overfitting, and Plasticity proxies (including Dormant neurons, representations rank, gradient norm, and parameters norm) with the resulting agent performance. These results indicate that these phenomena have a multifaceted influence on the final performance. However, the extent to which they interact varies between environments, and in particular, we notice a difference between simpler and more complex environments. \todo[inline]{To jest jeszcze do poprawy.}
    %Spearman correlation matrices reveal overestimation's strong correlation with agent returns, shedding light on critic regularization methods' limited robustness. Notably, Layer Norm and Spectral Norm emerge as effective mitigators of approximation errors, outperforming critic regularization methods, especially in specific setups. Regression tests deepen the analysis, uncovering that overestimation becomes a meaningful predictor of performance when fundamental issues like plasticity are addressed. The critic gradient norm stands out as a crucial metric, particularly in dog environments, suggesting a cascading nature of problems in reinforcement learning. \michalb{Multifacade - I wykrywamy problem input space na dogu}
\end{enumerate}


Specifically, GPL views the adjustment of pessimism as a dual optimization problem, resulting in the following update rule:

\begin{equation}
\label{eq:cetin_pessimism}
\begin{split}
    & \beta = \arg \min_{\beta} \underset{p_{0}, \pi}{\mathbb{E}} ~ \beta \left( Q^{\pi}(s,a) - r_{s,a} - \vartriangle \gamma V_{\phi}^{lb}(s') \right), \\
    & V_{\phi}^{lb}(s') \approx Q^{\mu}_{\phi}(s,a) - \beta Q^{\sigma}_{\phi}(s,a) - \alpha \log \pi_{\theta}(a|s).
\end{split}
\end{equation}


A different strategy, Tactical Optimism and Pessimism (\textbf{TOP}) \cite{moskovitz2021tactical}, adjusts pessimism using an external bandit controller to maximize online episodic rewards. However, this controller is discrete and less effective as the possible amount of pessimism values increases. 


\begin{figure*}[ht!]
\hspace{3cm}
	\begin{center}
			\begin{minipage}[h]{1.0\linewidth}     
   \centering
					\begin{subfigure}{0.9\linewidth}
							\includegraphics[width=0.49\linewidth]{icml2023/images/lineplots/dmc_rr2.png}
							\hfill
							\includegraphics[width=0.49\linewidth]{icml2023/images/lineplots/dmc_rr16.png}
						\end{subfigure}
				\end{minipage}
			\begin{minipage}[h]{1.0\linewidth}
        \centering
					\begin{subfigure}{0.9\linewidth}
							\includegraphics[width=0.49\linewidth]{icml2023/images/lineplots/mw_rr2.png}
							\hfill
							\includegraphics[width=0.49\linewidth]{icml2023/images/lineplots/mw_rr16.png}
						\end{subfigure}
				\end{minipage}
			\caption{
   Second-order results marginalizing critic regularization methods. On the x-axis, we have different types of plasticity regularization, and each color denotes network regularization. For better readability, points within one plasticity regularization are spaced slightly horizontally. Vertical lines indicate standard error.
   }
			\label{fig:marginalized}
		\end{center}
\end{figure*}

%We assess a model's performance across diverse problem domains to gauge its overall trainability.
%\begin{figure*}[ht!]
%	\begin{center}
%		\begin{minipage}[h]{1.0\linewidth}
%			\centering
%			\begin{subfigure}{0.75\linewidth}
%				\includegraphics[width=\textwidth]{icml2023/images/no_interaction/legend_no_interaction.png}
%			\end{subfigure}
%		\end{minipage}
%		\medskip
%		\begin{minipage}[h]{1.0\linewidth}
%			\begin{subfigure}{1.0\linewidth}
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Performance (RR=2).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Approximation Error (RR=2).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Overfitting (RR=2).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Dormant Neurons (RR=2).png}
%			\end{subfigure}
%		\end{minipage}
%		\begin{minipage}[h]{1.0\linewidth}
%			\begin{subfigure}{1.0\linewidth}
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Performance (RR=16).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Approximation Error (RR=16).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Overfitting (RR=16).png}
%				\hfill
%				\includegraphics[width=0.245\linewidth]{icml2023/images/no_interaction/Dormant Neurons (RR=16).png}
%			\end{subfigure}
%		\end{minipage}
%		\caption{.}
%		\label{fig:no_interaction}
%	\end{center}
%\end{figure*}

    %\item Critic regularization methods exhibit limited effectiveness in enhancing performance. When using network or plasticity regularization, critic regularization leads to reduced performance.
    %\item Periodical network resetting is the most robust intervention across two benchmarks in a high RR regime, and highly surpasses other plasticity regularization techniques in both robustness and performance.




% \begin{figure*}[ht!]
% 	\begin{center}
% 			\begin{minipage}[h]{1.0\linewidth}
% 					\begin{subfigure}{1.0\linewidth}
% 							\includegraphics[width=0.49\linewidth]{icml2023/images/interaction2/boxplots/dmc_rr2.png}
% 							\hfill
% 							\includegraphics[width=0.49\linewidth]{icml2023/images/interaction2/boxplots/dmc_rr16.png}
% 						\end{subfigure}
% 				\end{minipage}
% 			\begin{minipage}[h]{1.0\linewidth}
% 					\begin{subfigure}{1.0\linewidth}
% 							\includegraphics[width=0.49\linewidth]{icml2023/images/interaction2/boxplots/mw_rr2.png}
% 							\hfill
% 							\includegraphics[width=0.49\linewidth]{icml2023/images/interaction2/boxplots/mw_rr16.png}
% 						\end{subfigure}
% 				\end{minipage}
% 			\caption{DMC (top) MW (bottom).}
% 			\label{fig:marginalized}
% 		\end{center}
% \end{figure*}

%\mateusz{However, Dog has even higher gradients}

%Weight Decay or no Network Regularization makes most effective combinations with CRLU intervention (bottom-left plot in Figure~\ref{fig:marginalized}). For RR=16 (bottom-right plot in Figure~\ref{fig:marginalized}), the results align with first-order marginalization findings, highlighting the positive impact of Spectral Normalization. However, this type of marginalization reveals that SN works well with all plasticity regularization interventions except Resets, which work best without additional regularization or with Weight decay. For more details, see Appendix~\ref{app:Grad_analysis}.

%\begin{subfigure}{0.24\linewidth}
%        \includegraphics[width=0.93\linewidth]{icml2023/images/interventions/mw_rr=2_q_overestimation_eval.png}
%\end{subfigure}

%\begin{subfigure}{0.24\linewidth}
        %\includegraphics[width=0.93\linewidth]{icml2023/images/interventions/dmc_rr=2_q_overestimation_eval.png}
%\end{subfigure}

%\begin{figure}[ht!]
%	\begin{center}
%		\begin{minipage}[h]{1.0\linewidth}
%			\centering
%			\begin{subfigure}{0.93\linewidth}
%				\includegraphics[width=\textwidth]{icml2023/images/no_interaction/legend_no_interaction.png}
%			\end{subfigure}
%		\end{minipage}
%		\medskip
%		\begin{minipage}[h]{1.0\linewidth}
%			\begin{subfigure}{1.0\linewidth}
%				\includegraphics[width=0.49\linewidth]{icml2023/images/interventions/Grad Norm (RR=2) DMC.png}
%				\includegraphics[width=0.49\linewidth]{icml2023/images/interventions/Grad Norm (RR=16) DMC.png}
%			\end{subfigure}
%			\begin{subfigure}{1.0\linewidth}
%				\includegraphics[width=0.49\linewidth]{icml2023/images/interventions/Grad Norm (RR=2) MW.png}
%				\includegraphics[width=0.49\linewidth]{icml2023/images/interventions/Grad Norm (RR=16) MW.png}
%			\end{subfigure}
%		\end{minipage}
%		\caption{Interquantile Median Gradient Norm of First-Order Marginalization Over Timesteps. Results are presented for DMC (top row) and MW (bottom row) benchmarks, with columns representing replay ratios two (left) and sixteen (right).  Please refer to the color version for optimal viewing.}
%		\label{fig:GradNorms_timesteps}
%	\end{center}
%\end{figure}

%\begin{figure}[ht!]
%	\centering
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.95\linewidth]{icml2023/images/interventions/DMC_critic_gnorm_RR=2_IQM.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.95\linewidth]{icml2023/images/interventions/DMC_critic_gnorm_RR=16_IQM.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.95\linewidth]{icml2023/images/interventions/MW_critic_gnorm_RR=2_IQM.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.95\linewidth]{icml2023/images/interventions/MW_critic_gnorm_RR=16_IQM.png}
%	\end{subfigure}
%	\caption{IQM gradient norm of the top ten intervention pair combinations. The IQM is calculated based on the average of the last ten evaluation points in each run, not the last evaluation point.  Colors indicate hierarchy on the plot, not specific names.}
%	\label{fig:iqm-GradNorms}
%\end{figure}

%\subsection{Overestimation Analysis}
%\label{app:approx_error_analysis}
%\begin{figure}[ht!]
%	\centering
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.93\linewidth]{icml2023/images/interventions/dmc_rr=2_q_overestimation_eval.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.93\linewidth]{icml2023/images/interventions/dmc_rr=16_q_overestimation_eval.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.93\linewidth]{icml2023/images/interventions/mw_rr=2_q_overestimation_eval.png}
%	\end{subfigure}
%	\begin{subfigure}{0.24\linewidth}
%		\includegraphics[width=0.93\linewidth]{icml2023/images/interventions/mw_rr=16_q_overestimation_eval.png}
%	\end{subfigure}
%	\caption{IQM overestimation in logarithmic scale. Each plot presents sorted results. The IQM is calculated based on the average of the last ten evaluation points in each run, not the last evaluation point. Top row: DMC benchmark. Bottom row: MW. Colors indicate hierarchy on the plot, not specific names.}
%	%\label{fig:iqm-overestimation_1st_order}
%\end{figure}


% \begin{figure*}[ht!]
% \begin{center}
% \begin{minipage}[h]{1.0\linewidth}
%     \begin{subfigure}{1.0\linewidth}
%         \includegraphics[width=0.9\linewidth]{icml2023/images/interactions/metrics_2.png}
%     \end{subfigure}
% \end{minipage}
% \begin{minipage}[h]{1.0\linewidth}
%     \begin{subfigure}{1.0\linewidth}
%         \includegraphics[width=0.9\linewidth]{icml2023/images/interactions/metrics_16.png}
%     \end{subfigure}
% \end{minipage}
% \caption{.}
% \label{fig:task_specific_rr2}
% \end{center}
% \end{figure*}


% \begin{figure*}[ht!]
% \begin{center}
%     \begin{minipage}[h]{1.0\linewidth}
%         \begin{subfigure}{1.0\linewidth}
%             \includegraphics[width=0.99\linewidth]{icml2023/images/reg2/mw_regression_critic_gnorm_log_return_normalized_new_robust_False_one_row.png}
%         \end{subfigure}
%     \end{minipage}
% \caption{DMC (top) MW (bottom). Outliers perc=0.}
% \label{fig:mw_reg}
% \end{center}
% \end{figure*}




